Interpreting Criminal Charge Prediction and Its Algorithmic Bias via Quantum-Inspired Complex Valued Networks

While predictive policing has become increasingly common in assisting with decisions in the criminal justice system, the use of these results is still controversial. Some software based on deep learning lacks accuracy (e.g., in F-1), and importantly many decision processes are not transparent, causing doubt about decision bias, such as perceived racial and age disparities. This paper addresses bias issues with post-hoc explanations to provide a trustable prediction of whether a person will receive future criminal charges given one's previous criminal records by learning temporal behavior patterns over twenty years. Bi-LSTM relieves the vanishing gradient problem, attentional mechanisms allow learning and interpretation of feature importance, and complex-valued networks inspired quantum physics to facilitate a certain level of transparency in modeling the decision process. Our approach shows a consistent and reliable prediction precision and recall on a real-life dataset. Our analysis of the importance of each input feature shows the critical causal impact on decision-making, suggesting that criminal histories are statistically significant factors, while identifiers, such as race and age, are not. Finally, our algorithm indicates that a suspect tends to rather than suddenly increase crime severity level over time gradually.

==> sections/background.tex <==
\section{Background}

We train a support vector machine (SVM) model \cite{cortes1995support} with the radial basis function (RBF) kernel to build our baseline.

The feed-forward neural network we use has two hidden layers.
We use dropout \cite{srivastava2014dropout} for all the hidden layers.

We train a long short term memory (LSTM) network \cite{hochreiter1997long} for classification.
For each training sample, we feed the features one-by-one to the LSTM network.
Dropout is applied in the LSTM layers.
The output of the LSTM is fed to a linear layer which maps it to the number of target classes.
The initial hidden states of the LSTM are set to zeros.
Apart from using a unidirectional LSTM, we also train using a bidirectional LSTM.

Attention is a mechanism combined with recurrent networks, which allows it to focus on certain parts of the input sequence when predicting the output \cite{bahdanau2014neural}.
This enables better learning.
The combination of attention mechanisms enables improved performance in many tasks, making it an integral part of modern recurrent networks.
We apply attention with both unidirectional and bidirectional LSTMs.
Dropout is applied to the LSTM layers only, and the output is fed to a linear layer, which maps it to the number of target classes.
The initial hidden states of the network are set to zeros.

The neural network models explained above learn features and concepts in their hidden layers, making it hard to interpret them directly.
We use a recently proposed neural network based on the mathematical formulation of quantum physics.
Specifically, we train the quantum model proposed by \cite{li2019cnm}, which uses complex-valued vector space.
The original work by \cite{li2019cnm} proposed the quantum neural network model for the matching task.
However, we use this network for classification into the target classes directly.
Moreover, they used this model to train on text (natural language) data.
In our case, the training data consists of floating-point numbers as feature values.

% \begin{figure*}
%     \centering
%     \includegraphics[scale=0.08]{figures/cnm_model_drawio.pdf}
%     \caption{Modified CNM model}
%     \label{fig:cnm_model}
% \end{figure*}

More specifically, we build our modified CNM model (see figure \ref{fig:cnm_model}) as follows:
we first convert each feature to complex embeddings of size $d$.
An embedding layer with a ReLU activation \cite{nair2010rectified} takes as input the features one-by-one and converts them into two $d$-dimensional vectors, one for representing amplitude and the other for phase.
Each number in the phase embedding is normalized to fall in the range $[-\pi, \pi]$.

Given the complex embedding, we compute the relative weight of the $i$-th feature as the L2 norm of its amplitude.
We divide the amplitude by the L2 norm to get the new amplitude $A_i$.
Using this new amplitude $A_i$ and the phase $\phi_i$, we compute the real and imaginary parts of  $i$-th feature as follows:

\begin{equation}
    real_i = A_i\cos(\phi_i)
\end{equation}
\begin{equation}
    imag_i = A_i\sin(\phi_i)
\end{equation}

Let a training sample has $i = 1,\cdots, I$ features.
We model a training sample consisting of $I$ features using a local mixture scheme as in \cite{li2019cnm}.
The complex embeddings (comprising the amplitude and the phase) of the features are learned during the training process.

For all the neural network models, we use cross-entropy to calculate the loss.
The parameters are updated using the Adam optimizer \cite{kingma2014adam}.

\textcolor{red}{method}








